Spiking Neural Networks modelled as Timed Automata with parameter learning

In this paper we present a novel approach to automatically infer parameters of spiking neural networks. Neurons are modelled as timed automata waiting for inputs on a number of different channels (synapses), for a given amount of time (the accumulation period). When this period is over, the current potential value is computed considering current and past inputs. If this potential overcomes a given threshold, the automaton emits a broadcast signal over its output channel , otherwise it restarts another accumulation period. After each emission, the automaton remains inactive for a fixed refractory period. Spiking neural networks are formalised as sets of automata, one for each neuron, running in parallel and sharing channels according to the network structure. Such a model is formally validated against some crucial properties defined via proper temporal logic formulae. The model is then exploited to find an assignment for the synaptical weights of neural networks such that they can reproduce a given behaviour. The core of this approach consists in identifying some correcting actions adjusting synaptical weights and back-propagating them until the expected behaviour is displayed. A concrete case study is discussed.

==> abp_pseudocode.tex <==
% !TEX root = main.tex


%\begin{algorithm}[t]
%	\caption{Abstract \abp{}: Should Have Fired advice pseudo-code}
%	\label{alg.abp.shf}
%	\begin{algorithmic}[1]
%%		\Require $R \gg \Delta_W > \Delta_w$ \Comment{$R$ is the discretization granularity}
%		\Procedure{Should-Have-Fired}{$neuron$} 
%			\If{\Call{Is-Visited}{$neuron$}} 
%				\State \Return
%			\EndIf
%			\State \Call{Set-Visited}{$neuron$, True}
%			\Statex
%			\For{$i \gets 1\, \ldots\,$ \Call{Count-Predecessors}{$neuron$}} 
%				\State $weight_i \gets $ \Call{Get-Weight}{$neuron$, $i$}
%				\State $fired_i \gets $ \Call{Fired-Recently}{$neuron$, $i$}
%				\State $neuron_i \gets $ \Call{Get-Predecessor}{$neuron$, $i$}
%				\Statex
%			
%			\State \Call{Increase-Weight}{$neuron$, $i$, $\Delta$}
%				\Statex	
%				\If{$weight_i \geq 0$} 
%					\If{$ \neg fired_i$} 
%					
%						%\State \Call{Increase-Weight}{$neuron$, $i$, $\Delta$} \label{alg.abp.shf.smallstrengthen}
%						\State \Call{Should-Have-Fired}{$neuron_i$} \Comment{Advice propagation}
%					\EndIf 
%				\Else
%					\If{$fired_i$} 
%						%\State \Call{Increase-Weight}{$neuron$, $i$, $\Delta$} \label{alg.abp.shf.smallweaken}
%						\State \Call{Should-Not-Have-Fired}{$neuron_i$} \Comment{Advice propagation}
%					%\Else
%					%	\State \Call{Increase-Weight}{$neuron$, $i$, $\Delta$}
%					\EndIf 
%				\EndIf 
%			\EndFor
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}







\begin{algorithm}[t]
	\caption{Abstract \abp{}: Should \emph{Not} Have Fired advice pseudo-code}
	\label{alg.abp.snhf}
	\begin{algorithmic}[1]
	%	\Require $R \gg \Delta_W > \Delta_w$ \Comment{$R$ is the discretization granularity}
		\Procedure{Should-Not-Have-Fired}{$neuron$} 
			\If{\Call{Is-Visited}{$neuron$}} 
				\State \Return
			\EndIf
			\State \Call{Set-Visited}{$neuron$, True}
			\Statex
			\For{$i \gets 1\, \ldots\,$ \Call{Count-Predecessors}{$neuron$}} 
				\State $weight_i \gets $ \Call{Get-Weight}{$neuron$, $i$}
				\State $fired_i \gets $ \Call{Fired-Recently}{$neuron$, $i$}
				\State $neuron_i \gets $ \Call{Get-Predecessor}{$neuron$, $i$}
				\Statex
				\State \Call{Decrease-Weight}{$neuron$, $i$, $\Delta$}
				\Statex
				\If{$weight_i \geq 0$} 
					\If{$fired_i$} 
						%\State \Call{Decrease-Weight}{$neuron$, $i$, $\Delta_w$} \label{alg.abp.snhf.smallweaken}
						\State \Call{Should-Not-Have-Fired}{$neuron_i$} % \Comment{Advice propagation}
				%	\Else
						
					\EndIf 
				\Else
					\If{$ \neg fired_i$} 
				%		\State \Call{Decrease-Weight}{$neuron$, $i$, $\Delta$}
				%	\Else
						%\State \Call{Decrease-Weight}{$neuron$, $i$, $\Delta$} \label{alg.abp.snhf.smallstrengthen}
						\State \Call{Should-Have-Fired}{$neuron_i$} \Comment{Advice propagation}
					\EndIf 
				\EndIf 
			\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
